How Well Do Multi-modal LLMs Interpret CT Scans? An Auto-Evaluation Framework for Analyses

Automatically interpreting CT scans can ease the workload of radiologists. However, this is challenging mainly due to the scarcity of adequate datasets and reference standards for evaluation. This study aims to bridge this gap by introducing a novel evaluation framework, named ``GPTRadScore''. This framework assesses the capabilities of multi-modal LLMs, such as GPT-4 with Vision (GPT-4V), Gemini Pro Vision, LLaVA-Med, and RadFM, in generating descriptions for prospectively-identified findings. By employing a decomposition technique based on GPT-4, GPTRadScore compares these generated descriptions with gold-standard report sentences, analyzing their accuracy in terms of body part, location, and type of finding. Evaluations demonstrated a high correlation with clinician assessments and highlighted its potential over traditional metrics, such as BLEU, METEOR, and ROUGE. Furthermore, to contribute to future studies, we plan to release a benchmark dataset annotated by clinicians. Using GPTRadScore, we found that while GPT-4V and Gemini Pro Vision fare better, their performance revealed significant areas for improvement, primarily due to limitations in the dataset used for training these models. To demonstrate this potential, RadFM was fine-tuned and it resulted in significant accuracy improvements: location accuracy rose from 3.41\% to 12.8\%, body part accuracy from 29.12\% to 53\%, and type accuracy from 9.24\% to 30\%, thereby validating our hypothesis.

==> tmp.tex <==
Generating reports from volumetric data presents significant challenges and demands considerable resources, particularly in the identification of lesions, which usually represent only a small portion of the entire volume. This complexity is further amplified by the dual requirements of lesion detection and subsequent report generation. To effectively address this challenge, it is logical to decompose the complex task into two simpler, more manageable subtasks, as depicted in Figure \ref{fig:workflow}. The initial step involves the detection of lesions, followed by the application of vision-based LLMs for the generation of reports. Both of these components have been rigorously explored in existing literature and have demonstrated high levels of performance in their respective domains.

Nodule detection is a well-researched area, as evidenced by extensive literature \cite{hara2006nodule,zhang2018pulmonary,chillakuru2021high}, demonstrating significant success in achieving high accuracy. The pipeline is designed to incorporate any of these established models, thereby enabling the effective identification and delineation of nodules and/or areas of pathology. These models serve to highlight the pertinent slices of the scan, which are then processed as input for a vision-based LLM.

Vision-based LLM are specifically designed to interpret and generate textual information from visual data, making them particularly well-suited for the task of radiology report generation. The LLM receives the highlighted slices from the nodule detection module and generate detailed reports. While the reports generated are linguistically coherent, it is also imperative to evaluate them for clinical accuracy. To generate the final report for an entire volume, all reports corresponding to that volume are collated and further refined using a LLM.

Unlike the case with chest radiographs, for which a variety of automated methods for validating the clinical accuracy of reports have been established and detailed in several key studies \cite{wang2017chestx,peng2018negbio,irvin2019chexpert}, an equivalent automated system for the validation of clinical accuracy in CT reports is notably absent. Recently, Zhu et al. \cite{zhu2024leveraging} introduced an innovative evaluation framework that capitalizes on radiologists' domain expertise. This framework is designed to enhance LLM for the automatic evaluation of machine-generated radiology reports. This auto-evaluation method, combined with assessments conducted by trained radiologists, enables an expert review of the outputs from the vision-based LLM. This approach provides a comprehensive and clinically relevant analysis of the model's performance.
